CADS: A Systematic Literature Review on the Challenges of Abstractive Dialogue Summarization

Abstractive dialogue summarization is the task of distilling conversations into informative and concise summaries. Although reviews have been conducted on this topic, there is a lack of comprehensive work detailing the challenges of dialogue summarization, unifying the differing understanding of the task, and aligning proposed techniques, datasets, and evaluation metrics with the challenges. This article summarizes the research on Transformer-based abstractive summarization for English dialogues by systematically reviewing 1262 unique research papers published between 2019 and 2024, relying on the Semantic Scholar and DBLP databases. We cover the main challenges present in dialog summarization (i.e., language, structure, comprehension, speaker, salience, and factuality) and link them to corresponding techniques such as graph-based approaches, additional training tasks, and planning strategies, which typically overly rely on BART-based encoder-decoder models. We find that while some challenges, like language, have seen considerable progress, mainly due to training methods, others, such as comprehension, factuality, and salience, remain difficult and hold significant research opportunities. We investigate how these approaches are typically assessed, covering the datasets for the subdomains of dialogue (e.g., meeting, medical), the established automatic metrics and human evaluation approaches for assessing scores and annotator agreement. We observe that only a few datasets span across all subdomains. The ROUGE metric is the most used, while human evaluation is frequently reported without sufficient detail on inner-annotator agreement and annotation guidelines. Additionally, we discuss the possible implications of the recently explored large language models and conclude that despite a potential shift in relevance and difficulty, our described challenge taxonomy remains relevant.

==> content_text/072_conclusion.tex <==
\label{sec:conclusion}
In this article, we reviewed works on Transformer-based abstractive dialogue summarization.
We unified the existing definitions and concepts of dialogue summarization into a taxonomy (CADS) of the field's six main challenge blocks: language, structure, comprehension, speaker, salience, and reliability-related factuality.
We demonstrated how these challenges appear in dialogue summarization and discussed why they occur for established encoder-decoder-based summarization systems.
We then grouped and highlighted techniques introduced since 2019 under the challenges they tackle.
Despite advancements, we observed that the field is still in its infancy and offers ample opportunities for further research.
We also listed datasets used in existing studies to illustrate the extent of data scarcity in dialogue summarization. Additionally, we evaluated common metrics and noted a strong reliance on the ROUGE metric, coupled with a lack of human evaluation reports, which raises doubts about the actual effectiveness of current techniques.
In our discussion, we evaluated how current \gls{nlp} techniques address these challenges and derived implications of using \glspl{llm} for the field.
We thereby identify a lack of exploring such new models and borrowing effective techniques from related fields to overcome the limitations currently holding back progress.
We conclude that while challenges like language may become less relevant, others, such as comprehension and factuality, still require more exploration.
We recommend that future work should further discuss and adapt this taxonomy as new challenges, techniques, datasets, and evaluation measures emerge and as current challenges may be solved naturally through technological innovation.
The considered literature can be found in the accompanying repository\footnote{https://github.com/FKIRSTE/LitRev-DialogueSum \label{repository_link}} which will be regularly updated.


==> figures/challenges/categorization_of_subdomains.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.3]{figures/_storage/Organisation_of_Subdomains.png}
    \caption{Example image for a categorization. We can adopt this view and adapt it to our own ordering. This figure serves as an introduction and easy-to-grasp view on the sub-domains of dialogue summarization, while demonstrating how vanishing the boarders between the different dialogue types are. \textcolor{red}{The range would be from less structured to more structured dialogues.}}
    \label{fig:categorization_of_subdomains}
\end{figure*}

==> figures/challenges/dialogueVersusDocument.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.5]{figures/_storage/TempFigureDialogVsDoc.png}
    \caption{An example figure to show the challenge overlap between dialogue and document summarization. For demonstration, only challenge 1 is referenced here. There is no particular order to the challenges withing the circles.}
    \label{fig:dialogueVsDocument}
\end{figure*}

==> figures/datasets/dataset_challenge_matching.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/_storage/dataset_challenge_matching.png}
    \caption{Matching between established datasets and their primary reported challenge.}
    \label{fig:datasets_challenge_matching}
\end{figure}

==> figures/datasets/datasets_challenges.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/_storage/Dataset_Challenges.png}
    \caption{Overview of techniques and our taxonomy of the papers.}
    \label{fig:datasets_challenges}
\end{figure}

==> figures/datasets/datasets_overview.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/_storage/Datasets.png}
    \caption{Overview of established datasets in dialogue summarization, organized by the dialogue subdomain they reflect. For each dataset, we report a dataset card, including information about count, length, domain, characteristics, and link?}
    \label{fig:datasets_overview}
\end{figure}

==> figures/introduction/ExistingSurveys.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures//_storage/ExistingSurveys.png}
    \caption{Overview of existing surveys.}
    \label{fig:existing_surveys}
\end{figure}


==> figures/introduction/firstfigure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{example-image-a}
    \caption{First Figure.}
    \label{fig:firstfigure}
\end{figure}


==> figures/introduction/numberOfPapers.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.65]{figures/_storage/NumberOfPapers.png}
    \caption{<Placeholder> Annual number of papers related to abstractive dialogue summarization as considered in our review. Numbers for 2023 are low as this only counts papers until August 2023.}
    \label{fig:number_of_papers}
\end{figure*}

==> figures/methodology/papers_per_step.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.3]{figures/_storage/PaperFiltering.png}
    \caption{An overview of the paper filtering process. (1) denotes the total crawl, being 1000 papers from both Semantic Scholar and DBLP. Hence, half of the crawl are duplicates, marking section (2). Section (3) are papers excluded during the manual inspection based on the inclusion criteria described in X not being met in title or abstract, while additional works not meeting these criteria throughout the remainder of the paper making up section (4). This leaves section (5) with 130 paper being the ones that are considered in the literature review for the following sections.}
    \label{fig:papers_per_step}
\end{figure*}

==> figures/methodology/question_pipeline_classification.tex <==
\begin{figure*}
    \centering
    % \includegraphics[scale=0.8]{figures/_storage/question_pipeline_classification.png}
    \includegraphics[width=0.7\linewidth]{figures//_storage/tagging_pipeline.png}
    \caption{A placeholder of a question-pipeline to classify and tag papers. We adopted this with respective questions and will include it here.}
    \label{fig:question_pipeline_classification}
\end{figure*}


==> figures/techniques/model_overview.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures//_storage/model_overview.png}
    \caption{Model overview}
    \label{fig:model_overview}
\end{figure}

==> figures/techniques/taxonomy_techniques.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/_storage/ChallengesOverview.png}
    \caption{Overview of techniques and our taxonomy of the papers.}
    \label{fig:taxonomy_techniques}
\end{figure}

==> tables/Section_Challenges/papers_per_challenge_per_year.tex <==
\begin{table}[htbp]
\centering
% \begin{tabular}{lccccc}
% \toprule
% Challenge Family & 2019 & 2020 & 2021 & 2022 & 2023\\ 
% \midrule
% Language   & & & \cite{KhalifaBM21} & & \\
% Structure   & & & & & \\
% Understanding   & & & & & \\
% Speaker   & & & & & \\
% Data   & & & & & \\
% Salience   & & & & & \\
% Domain adaption   & & & & & \\
% sub-domains   & & & & & \\
% other   & & & & & \\
% \bottomrule
% \end{tabular}

\begin{tabularx}{\textwidth}{ lXXXXX }
  \toprule
  Challenge Family & 2019 & 2020 & 2021 & 2022 & 2023\\ 
  \midrule 
  Language   & & & \cite{KhalifaBM21} & & \\
  Understanding  & & & & & \\
  Speaker  & & & & & \\
  Data  & & & & & \\
  Salience  & & & & & \\
  Domain adaption  & & & & & \\
  sub-domains  & & & & & \\
  other  & & & & & \\
  \bottomrule
\end{tabularx}

\caption{Papers per challenge.}
\label{tab:papers_per_challenge_per_year}
\end{table}




==> tables/Section_Datasets/datasets_of_ds.tex <==
\begin{table}[tbp]
    \centering
    \begin{tabular}{l|c|c|c|c|c|c|c}
    \toprule
    Name & \#Samples & Avg. Length & \#Speakers & Topics & main challenge & Link  \\
    \midrule
    Daily Chat & x & x & x & x & x & x & x\\
    \midrule
    DialogSum & & & & & & & \\
    PersonaChat & & & & & & & \\
    MACSum & & & & & & & \\
    \midrule
    Online Chat & x & x & x & x & x & x & x\\
    \midrule
    DialogSum & & & & & & & \\
    PersonaChat & & & & & & & \\
    MACSum & & & & & & & \\
    \midrule
    Meeting & x & x & x & x & x & x & x\\
    \midrule
    DialogSum & & & & & & & \\
    PersonaChat & & & & & & & \\
    MACSum & & & & & & & \\
    \midrule
    Screenplay & x & x & x & x & x & x & x\\
    \midrule
    DialogSum & & & & & & & \\
    PersonaChat & & & & & & & \\
    MACSum & & & & & & & \\
    \midrule
    Customer Service & x & x & x & x & x & x & x\\
    \midrule
    DialogSum & & & & & & & \\
    PersonaChat & & & & & & & \\
    MACSum & & & & & & & \\
    \midrule
   Medical & x & x & x & x & x & x & x\\
    \midrule
    DialogSum & & & & & & & \\
    PersonaChat & & & & & & & \\
    MACSum & & & & & & & \\
    \midrule
    Debates & x & x & x & x & x & x & x\\
    \midrule
    DialogSum & & & & & & & \\
    PersonaChat & & & & & & & \\
    MACSum & & & & & & & \\
    \midrule
   Others & x & x & x & x & x & x & x\\
    \midrule
    DialogSum & & & & & & & \\
    PersonaChat & & & & & & & \\
    MACSum & & & & & & & \\
    \bottomrule
    \end{tabular}
    \caption{Open-domain dialogue summarization datasets. “AVL” refers to the public availability of the dataset (Y is available, N is not available, and C is conditional).}
    \label{tab:datasets_overview}
\end{table}

==> tables/Section_Evaluation/evaluation_summary.tex <==
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}


\begin{table}[t]
    \centering
    \footnotesize
    \setlength{\extrarowheight}{3pt} % Adds vertical space between rows
    \begin{tabular}{L{2.5cm} L{2cm} L{3cm} L{6cm} c}
        \toprule
        \textbf{Type} & \textbf{Category} & \textbf{Metric} & \textbf{Descriptive Tags} & \textbf{Usage} \\
        \midrule
        \multirow{1}{*}{Count-based} & N-gram & \textsc{Bleu} & overlap, precision, multiple references & 21 \\
        &  & \textsc{Rouge}  & word overlap, recall, one reference & 127 \\
        &  & \textsc{Meteor}  & word overlap, precision and recall, one reference & 3 \\
        &  & \textsc{ChrF++}  & character-level, F1 score, one reference & 2 \\
        &  & \textsc{Cider}  & consensus-based, multiple references & 3 \\
        \cline{2-5}
        & Statistical & \textsc{Perplexity} & likelihood of word sequences & 3 \\
        \midrule
        \multirow{1}{*}{Model-based} & Hybrid & \textsc{Bertscore} & token similarity, cosine similarity, one-to-one & 38 \\
        &  & \textsc{Moverscore} & token similarity, mover distance, one-to-many & 3 \\
        &  & \textsc{Factcc} & entailment classifier, scoring based on consistency & 9 \\
        \cline{2-5}
        & Trained & \textsc{Bleurt} & mimics human judgment & 7 \\
        &  & \textsc{Bartscore} & mimics human judgment, promptable & 13 \\
        &  & \textsc{Blanc} & fill-in-the-blank task with and without the summary & 2 \\
        \midrule
        \multirow{1}{*}{QA-based} & & \textsc{Feqa} & questions based on summary, answered through input & 38 \\
        &  & \textsc{Summaqa}  & questions based on input, answered through summary & 3 \\
        &  & \textsc{Questeval}  & combination of \textsc{Feqa} and \textsc{Summaqa} & 3 \\
        \midrule
        \multirow{1}{*}{\shortstack[l]{Human \\ Evaluation}} & Performance & \textsc{Likert Scale} & ordinal scale, e.g., 1 (worst) to 5 (best) & 6 \\
        &  & \textsc{Pairwise Comparison} & pick best sample out of two & 9 \\
        &  & \textsc{Best-Worst Scaling} & rank a list of samples & 5 \\
        \cline{2-5}
        & Agreement & \textsc{Krippendorff's Alpha} & measure disagreement, different data formats & 2 \\
        &  & \textsc{Cohen's Kappa} & measure agreements, categorical data, 2 raters & 3 \\
        &  & \textsc{Fleiss' Kappa} & measure agreement, nominal data, 2 raters & 2 \\
        \bottomrule
    \end{tabular}
    \caption{Relevant metrics and evaluation measures employed in dialogue summarization with more than twice reported use. `Usage' states the number of papers reporting the evaluation measure in their publication.}
    \label{tab:evaluation_summary}
\end{table}

% \begin{table}[]
%     \centering
%     \small
%     \begin{tabular}{L{1.5cm} L{2cm} L{3.5cm} L{6cm} c}
%         \toprule
%         \textbf{Type} & \textbf{Category} & \textbf{Metric} & \textbf{Descriptive Tags} & \textbf{Usage} \\
%         \midrule
%         Count-based & N-gram & \textsc{Bleu} & word overlap, precision, multiple references & 21 \\
%         &  & \textsc{Rouge}  & word overlap, recall, one reference & 127 \\
%         &  & \textsc{Meteor}  & word overlap, precision and recall, one reference & 3 \\
%         &  & \textsc{ChrF++}  & character-level, F1 score, one reference & 2 \\
%         &  & \textsc{Cider}  & consensus-based, multiple references & 3 \\
%         \hdashline
%         &  Statistical & \textsc{Perplexity}  & likelihood of word sequences & 3 \\
%         \midrule
%         Model-based & Hybrid & \textsc{Bertscore}  & token similarity, cosine-similarity, one-to-one & 38 \\
%         &  & \textsc{Moverscore}  & token similarity, mover distance, one-to-many & 3 \\
%         &   & \textsc{Factcc}  & entailment classifier, scoring based on consistency & 9 \\
%         \hdashline
%         &  Trained & \textsc{Bleurt}  & mimics human judgement & 7 \\
%         &   & \textsc{Bartscore}  & mimics human judgement, promptable & 13 \\
%         &   & \textsc{Blanc}  & fill-in-the-blank task with and without the summary & 2 \\
%         \midrule
%         QA-based & & \textsc{Feqa} & questions based on summary, answered through input & 38 \\
%         &  & \textsc{Summaqa}  & questions based on input, answered through summary & 3 \\
%         &  & \textsc{Questeval}  & combination of \textsc{Feqa} and \textsc{Summaqa} & 3 \\
%         \midrule
%         Human Evaluation & Performance & \textsc{Likert Scale} & scale, typically 1 (worst) to 5 (best) & 6 \\
%         &  & \textsc{Pairwise Comparison} & pick best sample out of two & 9 \\
%         &  & \textsc{Best-Worst Scaling} & rank a list of samples & 5 \\
%         \hdashline
%         &  Agreement & \textsc{Krippendorff's Alpha} & measure disagreement, different data formats & 2 \\
%         &   & \textsc{Cohen's Kappa} & measure agreements, categorical data, 2 raters & 3 \\
%         &   & \textsc{Fleiss' Kappa} & measure agreement, nominal data, 2 raters & 2 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Relevant metrics and evaluation measures employed in dialogue summarization with more than twice reported use. 'Usage' states the number of papers reporting the evaluation measure in their publication.}
%     \label{tab:evaluation_summary}
% \end{table}

% \begin{table}[]
%     \centering
%     \small
%     \begin{tabular}{L{1.5cm} L{1.5cm} L{2cm} L{6cm} c}
%         \toprule
%         \textbf{Type} & \textbf{Category} & \textbf{Metric} & \textbf{Descriptive Tags} & \textbf{Usage} \\
%         \midrule
%         Count-based & N-gram & BLEU & word overlap, precision, multiple references & 21 \\
%         &  & ROUGE  & word overlap, recall, one reference & 127 \\
%         &  & METEOR  & word overlap, precision and recall, one reference & 3 \\
%         &  & chrF++  & character-level, F1 score, one reference & 2 \\
%         &  & CIDEr  & consensus-based, multiple references & 3 \\
%         \hdashline
%         &  Statistical & Perplexity  & likelihood of word sequences & 3 \\
%         \midrule
%         Model-based & Hybrid & BERTScore  & token similarity, cosine-similarity, one-to-one & 38 \\
%         &  & MoverScore  & token similarity, mover distance, one-to-many & 3 \\
%         &   & FactCC  & entailment classifier, scoring based on consistency & 9 \\
%         \hdashline
%         &  Trained & BLEURT  & mimics human judgement & 7 \\
%         &   & BARTScore  & mimics human judgement, promptable & 13 \\
%         &   & BLANC  & fill-in-the-blanc task with and without the summary & 2 \\
%         \midrule
%         QA-based & & FEQA & questions based on summary, answered through input & 38 \\
%         &  & SummaQA  & questions based on input, answered through summary & 3 \\
%         &  & QuestEval  & combination of FEQA and SummQA & 3 \\
%         \midrule
%         Human Evaluation & Performance & Likert Scale & scale, typically 1 (worst) to 5 (best) & 6 \\
%         &  & Pairwise Comparison & pick best sample out of two & 9 \\
%         &  & Best-Worst Scaling & rank a list of samples & 5 \\
%         \hdashline
%         &  Agreement & Krippendorff's Alpha & measure disagreement, different data formats & 2 \\
%         &   & Cohen's Kappa & measure agreements, categorical data, 2 raters & 3 \\
%         &   & Fleiss' Kappa & measure agreement, nominal data, 2 raters & 2 \\
%         %&   & Pearson Correlation \cite{PearsonG95} & measure agreement, linear correlation assumed & 2 \\
%         %&   & Spearman Correlation \cite{Spearman04a} & measure agreement, monotonic relationship & 4 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Relevant metrics and evaluation measures employed in dialogue summarization with more than twice reported use. 'Usage' states the number of papers reporting the evaluation measure in their publication.}
%     \label{tab:evaluation_summary}
% \end{table}

% \begin{table}[]
%     \centering
%     \small
%     \begin{tabular}{L{1.5cm} L{1.5cm} L{2cm} L{6cm} c}
%         \toprule
%         \textbf{Type} & \textbf{Category} & \textbf{Metric} & \textbf{Descriptive Tags} & \textbf{Usage} \\
%         \midrule
%         Count-based & N-gram & BLEU \cite{PapineniRWZ02} & word overlap, precision, multiple references & 21 \\
%         &  & ROUGE \cite{Lin04} & word overlap, recall, one reference & 127 \\
%         &  & METEOR \cite{BanerjeeL05} & word overlap, precision and recall, one reference & 3 \\
%         &  & chrF++ \cite{Popovic17} & character-level, F1 score, one reference & 2 \\
%         &  & CIDEr \cite{VedantamZP15} & consensus-based, multiple references & 3 \\
%         \hdashline
%         &  Statistical & Perplexity \cite{JelinekMBB77} & likelihood of word sequences & 3 \\
%         \midrule
%         Model-based & Hybrid & BERTScore \cite{ZhangKWW20a} & token similarity, cosine-similarity, one-to-one & 38 \\
%         &  & MoverScore \cite{ZhaoPLG19} & token similarity, mover distance, one-to-many & 3 \\
%         &   & FactCC \cite{KryscinskiMXS20a} & entailment classifier, scoring based on consistency & 9 \\
%         \hdashline
%         &  Trained & BLEURT \cite{SellamDP20} & mimics human judgement & 7 \\
%         &   & BARTScore \cite{YuanNL21} & mimics human judgement, promptable & 13 \\
%         &   & BLANC \cite{VasilyevDB20a} & fill-in-the-blanc task with and without the summary & 2 \\
%         \midrule
%         QA-based & & FEQA \cite{DurmusHD20a} & questions based on summary, answered through input & 38 \\
%         &  & SummaQA \cite{ScialomLPS19} & questions based on input, answered through summary & 3 \\
%         &  & QuestEval \cite{DeutschBR21} & combination of FEQA and SummQA & 3 \\
%         \midrule
%         Human Evaluation & Performance & Likert Scale \cite{Likert32a} & scale, typically 1 (worst) to 5 (best) & 6 \\
%         &  & Pairwise Comparison \cite{ElderGOL18} & pick best sample out of two & 9 \\
%         &  & Best-Worst Scaling \cite{FinnL92} & rank a list of samples & 5 \\
%         \hdashline
%         &  Agreement & Krippendorff's Alpha \cite{Krippendorff70} & measure disagreement, different data formats & 2 \\
%         &   & Cohen's Kappa \cite{Cohen60} & measure agreements, categorical data, 2 raters & 3 \\
%         &   & Fleiss' Kappa \cite{Fleiss71a} & measure agreement, nominal data, 2 raters & 2 \\
%         %&   & Pearson Correlation \cite{PearsonG95} & measure agreement, linear correlation assumed & 2 \\
%         %&   & Spearman Correlation \cite{Spearman04a} & measure agreement, monotonic relationship & 4 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Relevant metrics and evaluation measures employed in dialogue summarization with more than twice reported use. 'Usage' states the number of papers reporting the evaluation measure in their publication.}
%     \label{tab:evaluation_summary}
% \end{table}


% \begin{figure}
%     \centering
%     \includegraphics[scale=1]{example-image-c} 
%     \caption{Evaluation measures used in dialogue summarization. "Used" marks the number of papers that consider the metric in their publication in our 130 filtered literature crawl. <This should serve as brief summary and NOT as replacement to the text>.}
%     \label{tab:evaluation_summary}
% \end{figure}

==> tables/Section_Introduction/different_challenge_interpretation.tex <==
\begin{table}[tbp]
    \centering
    \begin{tabularx}{\textwidth}{lXc}
    \toprule
    Challenge & Definition & Reference  \\
    \midrule
    Speaker Dynamics & A & \Cref{missing_citation} \\
    Speaker Dynamics & B & \Cref{missing_citation} \\
    \bottomrule
    \end{tabularx}
    \caption{Example of subtly different challenge definitions in current works.}
    \label{tab:different_challenge_definitions_example}
\end{table}

==> tables/progress/challenges_paper_breakdown.tex <==
\begin{table}[]
    \centering
    \small
    \begin{tabularx}{\textwidth}{lXXccc}
    \toprule
    Challenge & Description & Sub-Challenge & \# Char. & \# Tech. & \#Total\\
    \midrule
    Language & Idiosyncratic nature of spoken language and individual speech patterns. & Linguistic Subtleties \textit{(e.g., informality, grammaticality, colloquialism)} & 4 & 8 & 10 \\
    & & Content Repetition \textit{(e.g., restarts)} & -1 & -1 & -1 \\
    & & Domain-Specific Terminology \textit{(e.g., medical terms)} & -1 & -1 & -1 \\
    \midrule
    Salience & & & & & \\
    & & & & & \\
    & & & & & \\
    \midrule
    Structure & & & & & \\
    & & & & & \\
    & & & & & \\
    \midrule
    Understanding & & & & & \\
    & & & & & \\
    & & & & & \\
    \midrule
    Language & & & & & \\
    & & & & & \\
    & & & & & \\
    \midrule 
    Factuality & & & & & \\
    & & & & & \\
    & & & & & \\
    \midrule
    $\Sigma$ & & & 94 & 97 & 100 \\
    \bottomrule
    \end{tabularx}
    \caption{A breakdown of the number of papers per challenge and per sub-challenge considering the characteristics, techniques, and in total (de-duplicated).}
    \label{tab:challenges_number_papers}
\end{table}


        %  \toprule
        %  Challenge & \# Characterizing papers & \# Technique papers & \#total\\
        %  \midrule
        %  Language & \begin{tabular}{@{}l@{}} Style: 4 \\ Negation: 1 \\ Repetition: 1\end{tabular} & \begin{tabular}{@{}l@{}} Style: 8 \\ Negation: 1 \\ 
        %  Repetition: 1\end{tabular} & 10 \\
        %  \midrule
        %  Structural & \begin{tabular}{@{}l@{}} Topic: 5 \\ Phase: 4 \\ Utterance: 8\end{tabular} & \begin{tabular}{@{}l@{}} Topic: 6 \\ Phase: 3 \\ 
        %  Utterance: 7\end{tabular} & 16 \\
        %  \midrule
        %  Understanding & \begin{tabular}{@{}l@{}} Context: 2\end{tabular} & \begin{tabular}{@{}l@{}} Context: 1\end{tabular} & 1 \\
        %  \midrule
        %  Speaker & \begin{tabular}{@{}l@{}} Dynamics: 20 \\ Role: 5? \\ Co-reference: 7\end{tabular} & \begin{tabular}{@{}l@{}} Dynamics: 12 \\ Role: 5 \\ Co-reference: 7\end{tabular} & 24\\
        %  \midrule
        %  Salience & \begin{tabular}{@{}l@{}} Determination: 3 \\ Location: 5 \end{tabular} & \begin{tabular}{@{}l@{}} Determination: 12 \\ Location: 3\end{tabular} & 15 \\
        %  \midrule
        %  Data & \begin{tabular}{@{}l@{}} Scarcity: 10? (3+7)\end{tabular} & \begin{tabular}{@{}l@{}} Scarcity: 8\end{tabular} & 8 \\
        % \midrule
        % $\Sigma$ & & 74 \\
        % \bottomrule
